What Can We Learn from Harry Potter? An Exploratory Study of Visual Representation Learning from Atypical Videos

Humans usually show exceptional generalisation and discovery ability in the open world, when being shown uncommon new concepts. Whereas most existing studies in the literature focus on common typical data from closed sets, open-world novel discovery is under-explored in videos. In this paper, we are interested in asking: What if atypical unusual videos are exposed in the learning process? To this end, we collect a new video dataset consisting of various types of unusual atypical data (e.g., sci-fi, animation, etc.). To study how such atypical data may benefit open-world learning, we feed them into the model training process for representation learning. Focusing on three key tasks in open-world learning: out-of-distribution (OOD) detection, novel category discovery (NCD), and zero-shot action recognition (ZSAR), we found that even straightforward learning approaches with atypical data consistently improve performance across various settings. Furthermore, we found that increasing the categorical diversity of the atypical samples further boosts OOD detection performance. Additionally, in the NCD task, using a smaller yet more semantically diverse set of atypical samples leads to better performance compared to using a larger but more typical dataset. In the ZSAR setting, the semantic diversity of atypical videos helps the model generalise better to unseen action classes. These observations in our extensive experimental evaluations reveal the benefits of atypical videos for visual representation learning in the open world, together with the newly proposed dataset, encouraging further studies in this direction. The project page is at: https://julysun98.github.io/atypical_dataset.

==> Figure/OOD_ablation_class.tex <==
\begin{figure*}[htb]
    \centering
    % 第一个子图
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/fpr95_ablation.pdf}
        \caption{EPR95(↓) performance.}
        \label{fig:subfig1}
    \end{subfigure}
    % \hfill
    \hspace{0.02\textwidth}
    % 第二个子图
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/auc_ablation.pdf}
        \caption{AUROC(↑) performance.}
        \label{fig:subfig2}
    \end{subfigure}
    % \hfill
    \hspace{0.02\textwidth}
    % 第三个子图
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figure/aupr_ablation.pdf}
        \caption{AUPR(↑) performance.}
        \label{fig:subfig3}
    \end{subfigure}
    \vspace{-1em}
    \caption{Result of the effect of the number of categories of atypical data on the performance of OOD detection. atypical-n corresponds to the results for n categories in atypical outlier exposure data only, respectively. \textcolor{blue}{is it an incremental combination?}}
    \label{fig:OOD_ablation_class}
\vspace{-1em}
\end{figure*}

==> Table/OOD_main.tex <==
% \begin{table}[htbp]
%     \centering
%     \small
%     \caption{OOD detection performance of models trained with various auxiliary outlier datasets, including Gaussian noise, Diving48, K400, and the proposed atypical dataset(FPR95↓, AUROC↑, AUPR↑). Baseline is trained using only ID data UCF101. The best results are highlighted in \textbf{bold}.}% +X denotes a model that introduces an auxiliary dataset X for training."Mean" represents the averaged results across all new data ($D_{out}$).
%     % \resizebox{\columnwidth}{!}{
%     \vspace{1em}
%     \begin{tabular}{c|cccc}
%         \toprule
%         \textbf{new data: $D_{out}$} & \textbf{aux data} & \textbf{FPR95 ↓} & \textbf{AUROC ↑} & \textbf{AUPR ↑} \\
%         \midrule
%      %    \multirow{5}{*}{Bernolli\\ Noise} & Baseline & 14.57 & 90.11 & 45.39 \\
%      % & +Gaussian & \textbf{0.00} & \textbf{100.00} & \textbf{0.00} \\
%      % & +diving48 & 6.64 & 95.60 & 63.53 \\
%      % & +K400 & 15.26 & 87.56 & 40.26 \\
%      % & +\textit{atypical} & 7.16 & 94.82 & 59.84 \\
%      %    \midrule
%     \multirow{5}{*}{HMDB51} & Baseline & 77.08 & 63.85 & 22.54 \\
%      & +Gaussian & 81.11 & 63.36 & 23.03 \\
%      & +Diving48 & 81.14 & 64.84 & 24.04 \\
%      & +K400 & 75.52 & 66.84 & 25.13 \\
%      & +\textit{atypical} & \textbf{73.07} & \textbf{69.43} & \textbf{27.07} \\
%         \midrule
%  \multirow{5}{*}{MiT-v2} & Baseline & 77.73 & 64.94 & 23.76 \\
%      & +Gaussian & 77.51 & 65.14 & 24.12 \\
%      & +Diving48 & 80.87 & 65.46 & 27.24 \\
%       & +K400 & 67.72 & 72.53 & 30.86 \\
%  & +\textit{atypical} & \textbf{66.62} & \textbf{74.01} & \textbf{32.59} \\
%         \midrule
% \multirow{5}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\ -surreal}}
%  & Baseline & 62.22 & 75.50 & 33.42 \\
%   & +Gaussian & 67.37 & 73.32 & 32.26 \\
%   & +Diving48 & 73.14 & 69.13 & 25.71 \\
% & +K400 & 53.66 & 79.78 & 39.13 \\
%  & +\textit{atypical} & \textbf{49.99} & \textbf{82.03} & \textbf{43.19}\\
%         \midrule
% \multirow{5}{*}
% {\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-theatre }}& Baseline & 79.75 & 61.80 & 20.34 \\
%    & +Gaussian & 80.71 & 63.95 & 21.97 \\
%  & +Diving48 & 82.66 & 60.05 & 19.04 \\
%   & +K400 & 66.41 & 71.29 & 27.17 \\
%  & +\textit{atypical} & \textbf{61.91} & \textbf{74.62} & \textbf{34.57} \\
%         % \midrule
%         % Mean & Baseline & 74.20 & 66.52 & 25.02 \\
%         %      & +Gaussian & 76.68 & 66.44 & 25.25 \\
%         %      & +diving48 & 79.45 & 64.87 & 24.01 \\
%         %      & +K400 & 65.83 & 72.61 & 30.57 \\
%         %      & +\textit{atypical} & \textbf{62.90} & \textbf{75.02} & \textbf{34.36} \\
%         \bottomrule
%     \end{tabular}
%     % }
%     \vspace{-3em}
% \label{tab:OOD_main}
% \end{table}
\begin{table}[h]
\centering
\small
\caption{OOD detection performance using different auxiliary datasets with a ResNet3D-50 backbone. Results are reported on four test sets: HMDB51, MiT-v2, [\textit{atypical}]-surreal, and [\textit{atypical}]-theatre. \textit{Baseline}: training w/o auxiliary data; the others add auxiliary data. The best results are highlighted in \textbf{bold}.}

\vspace{1em}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|l|ccccc}
\toprule
\textbf{Dataset} & \textbf{Metric} & Baseline & +Gaussian & +Diving48 & +K400 & +\textit{Atypical} \\
\midrule
\multirow{3}{*}{HMDB51}
& FPR95 ↓ & 77.08 & 81.11 & 81.14 & 75.52 & \textbf{73.07} \\
& AUROC ↑ & 63.85 & 63.36 & 64.84 & 66.84 & \textbf{69.43} \\
& AUPR ↑  & 22.54 & 23.03 & 24.04 & 25.13 & \textbf{27.07} \\
\midrule
\multirow{3}{*}{MiT-v2}
& FPR95 ↓ & 77.73 & 77.51 & 80.87 & 67.72 & \textbf{66.62} \\
& AUROC ↑ & 64.94 & 65.14 & 65.46 & 72.53 & \textbf{74.01} \\
& AUPR ↑  & 23.76 & 24.12 & 27.24 & 30.86 & \textbf{32.59} \\
\midrule
\multirow{3}{*}{[\textit{atypical}]-surreal}
& FPR95 ↓ & 62.22 & 67.37 & 73.14 & 53.66 & \textbf{49.99} \\
& AUROC ↑ & 75.50 & 73.32 & 69.13 & 79.78 & \textbf{82.03} \\
& AUPR ↑  & 33.42 & 32.26 & 25.71 & 39.13 & \textbf{43.19} \\
\midrule
\multirow{3}{*}{[\textit{atypical}]-theatre}
& FPR95 ↓ & 79.75 & 80.71 & 82.66 & 66.41 & \textbf{61.91} \\
& AUROC ↑ & 61.80 & 63.95 & 60.05 & 71.29 & \textbf{74.62} \\
& AUPR ↑  & 20.34 & 21.97 & 19.04 & 27.17 & \textbf{34.57} \\
\bottomrule
\end{tabular}
\vspace{-1em}
\label{tab:OOD_main}
\end{table}


==> Table/OOD_mean.tex <==
% \begin{table}[htbp]
%     \centering
%     \small
%     \caption{Average OOD detection performance (FPR95 ↓, AUROC ↑, AUPR ↑) using different auxiliary datasets during training. All models are evaluated on four test sets: HMDB51, MiT-v2, [\textit{atypical}]-surreal, and [\textit{atypical}]-theatre. The best results are highlighted in \textbf{bold}.}.
%     % \caption{OOD detection performance of models trained with various auxiliary outlier datasets, including Gaussian noise, Diving48, K400, and the proposed atypical dataset(FPR95↓, AUROC↑, AUPR↑). Baseline is trained using only ID data UCF101. The best results are highlighted in \textbf{bold}.}% +X denotes a model that introduces an auxiliary dataset X for training."Mean" represents the averaged results across all new data ($D_{out}$).
%     % \resizebox{\columnwidth}{!}{
%     \vspace{2em}
%     \begin{tabular}{c|l|ccc}
%         \toprule
%         \textbf{new data: $D_{out}$} & \textbf{aux data} & \textbf{FPR95 ↓} & \textbf{AUROC ↑} & \textbf{AUPR ↑} \\
%         \midrule
%      %    \multirow{5}{*}{Bernolli\\ Noise} & Baseline & 14.57 & 90.11 & 45.39 \\
%      % & +Gaussian & \textbf{0.00} & \textbf{100.00} & \textbf{0.00} \\
%      % & +diving48 & 6.64 & 95.60 & 63.53 \\
%      % & +K400 & 15.26 & 87.56 & 40.26 \\
%      % & +\textit{atypical} & 7.16 & 94.82 & 59.84 \\
%      %    \midrule
%     \multirow{5}{*}{Mean} & Baseline & 74.20 & 66.52 & 25.02 \\
%      & +Gaussian & 76.68 & 66.44 & 25.35 \\
%      & +Diving48 & 79.45 & 64.87 & 24.01 \\
%      & +K400 & 65.83 & 72.61 & 30.62 \\
%      & +\textit{atypical} & \textbf{62.90} & \textbf{75.02} & \textbf{34.36} \\
%         \bottomrule
%     \end{tabular}
%     % }
%     \vspace{-1em}
% \label{tab:OOD_mean}
% \end{table}

\begin{table}[htbp]
    \centering
    \small
    % \caption{Average OOD detection performance (FPR95 ↓, AUROC ↑, AUPR ↑) using different auxiliary datasets during training. All models are evaluated on four test sets: HMDB51, MiT-v2, [\textit{atypical}]-surreal, and [\textit{atypical}]-theatre. The best results are highlighted in \textbf{bold}.Detailed results on each test dataset (HMDB51, MiT-v2, [\textit{atypical}]-surreal, and [\textit{atypical}]-theatre) are provided in the supplementary material.}
    \caption{Average OOD performance (FPR95 ↓, AUROC ↑, AUPR ↑) using different auxiliary datasets during training. All models are evaluated on four testsets: HMDB51, MiT-v2, [\textit{atypical}]-surreal, and [\textit{atypical}]-theatre. \textit{Baseline}: training w/o auxiliary data. Best results are shown in \textbf{bold}. Detailed results per test set are provided in the supplementary material.}
    \vspace{1em}
    \begin{tabular}{l|ccccc}
        \toprule
        \textbf{Metric} & Baseline & +Gaussian & +Diving48 & +K400 & +\textit{atypical} \\
        \midrule
        FPR95 ↓ & 74.20 & 76.68 & 79.45 & 65.83 & \textbf{62.90} \\
        AUROC ↑ & 66.52 & 66.44 & 64.87 & 72.61 & \textbf{75.02} \\
        AUPR ↑ & 25.02 & 25.35 & 24.01 & 30.62 & \textbf{34.36} \\
        \bottomrule
    \end{tabular}
    % \vspace{-1em}
\label{tab:OOD_mean}
\end{table}


==> Table/ablation_OOD1_.tex <==
% \begin{table}[htbp]
% \centering
% \caption{OOD detection performance with the introduction of any one category of \textit{atypical} data. The best results are highlighted in \textbf{bold}.}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|c|cccc}
% \hline
% \makecell{new data:\\$D_{out}$} & Metric & +$OE_{abn}$ &  +$OE_{ani}$  & +$OE_{sci}$ & +$OE_{uni}$\\
% \hline
% % \multirow{3}{*}{\makecell[c]{Gaussian \\ Noise}}  
% % & FPR95 ↓ & 13.33 & 36.44 & 22.56 & \textbf{8.97} \\
% % & AUROC ↑ & 88.54 & 67.34 & 81.61 & \textbf{92.13} \\
% % & AUPR ↑  & 41.97 & 21.66 & 31.80 & \textbf{50.31} \\
% % \hline
% % \multirow{3}{*}{\makecell[c]{Bernoulli \\Noise}} 
% % & FPR95 ↓ & 26.61 & 66.58 & 53.13 & \textbf{8.05} \\
% % & AUROC ↑ & 80.78 & 36.01 & 52.37 & \textbf{93.42} \\
% % & AUPR ↑  & 30.84 & 12.92 & 16.24 & \textbf{54.28} \\
% % \hline
% \multirow{3}{*}{HMDB51} 
% & FPR95 ↓ & \underline{84.41} & 80.41 & \textbf{79.06} & 81.29 \\
% & AUROC ↑ & \underline{60.81} & 67.01 & \textbf{68.14} & 66.05 \\
% & AUPR ↑  & \underline{21.73} & 28.09 & \textbf{32.36} & 23.84 \\
% \hline
% \multirow{3}{*}{MiT-v2} 
% & FPR95 ↓ & \underline{83.63} & 75.75 & 81.93 & \textbf{61.05} \\
% & AUROC ↑ & \underline{61.98} & 66.86 & 62.85 & \textbf{74.39} \\
% & AUPR ↑  & \underline{22.98} & 25.42 & 23.45 & \textbf{31.48} \\
% \hline
% \multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-surreal}} 
% & FPR95 ↓ & \underline{75.52} & 69.46 & 75.43 & \textbf{41.80} \\
% & AUROC ↑ & 66.78 & 69.86 & \underline{66.41} & \textbf{84.93} \\
% & AUPR ↑  & 24.34 & 25.85 & \underline{24.25} & \textbf{47.11} \\
% \hline
% \multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-theatre }}
% & FPR95 ↓ & \underline{88.53} & \textbf{40.78} & 67.05 & 70.75 \\
% & AUROC ↑ & \underline{53.71} & \textbf{89.66} & 78.73 & 59.29 \\
% & AUPR ↑  & \underline{16.60} & \textbf{64.97} & 48.42 & 17.45 \\
% \hline
% % \multirow{3}{*}{Mean} 
% % & FPR95 ↓ & 52.00 & 64.80 & 59.17 & \textbf{39.84} \\
% % & AUROC ↑ & 73.03 & 59.30 & 66.24 & \textbf{81.50} \\
% % & AUPR ↑  & 29.38 & 22.02 & 25.96 & \textbf{39.98} \\
% % \hline
% \end{tabular}}
% \label{tab:ood1}
% \end{table}

% \vspace{-1em}
\begin{table}[htbp]
\centering
\small
\caption{OOD detection performance with the introduction of any one category of \textit{atypical} data. + indicates the introduction of auxiliary \textit{atypical} data.  $abn$ denotes [\textit{atypical}]-{abnormal}, $ani$ denotes [\textit{atypical}]-animation, $sci$ denotes [\textit{atypical}]-sci-fi, and $uni$ denotes [\textit{atypical}]-unintentional. The best results per metric are highlighted in \textbf{bold}, and the second-best results are \underline{underlined}.}
\vspace{1em}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|cccc|c}
\hline
\makecell{Test sets} & Metric & +$abn$ &  +$ani$  & +$sci$ & +$uni$ & \makecell{Mean ± Std Dev}\\
\hline
\multirow{3}{*}{\shortstack{{HMDB51}\\~\cite{kuehne2011hmdb}}}  
& FPR95 ↓ & 84.41 & \underline{80.41} & \textbf{79.06} & 81.29 & 81.29\pm2.27 \\
& AUROC ↑ & 60.81 & \underline{67.01} & \textbf{68.14} & 66.05 & 65.50\pm3.24 \\
& AUPR ↑  & 21.73 & \underline{28.09} & \textbf{32.36} & 23.84 & 26.50\pm4.71 \\
\hline
\multirow{3}{*}{
\shortstack{{MiT-v2}\\~\cite{monfort2019moments}}}
& FPR95 ↓ & 83.63 & \underline{75.75} & 81.93 & \textbf{61.05} & 75.59\pm10.27 \\
& AUROC ↑ & 61.98 & \underline{66.86} & 62.85 & \textbf{74.39} & 66.52\pm5.66 \\
& AUPR ↑  & 22.98 & \underline{25.42} & 23.45 & \textbf{31.48} & 25.83\pm3.91 \\
\hline
\multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-surreal}} 
& FPR95 ↓ & 75.52 & \underline{69.46} & 75.43 & \textbf{41.80} & 65.55\pm16.09 \\
& AUROC ↑ & 66.78 & \underline{69.86} & 66.41 & \textbf{84.93} & 72.00\pm8.76 \\
& AUPR ↑  & 24.34 & \underline{25.85} & 24.25 & \textbf{47.11} & 30.39\pm11.17 \\
\hline
\multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-theatre}} 
& FPR95 ↓ & 88.53 & \textbf{40.78} & \underline{67.05} & 70.75 & 66.78\pm19.71 \\
& AUROC ↑ & 53.71 & \textbf{89.66} & \underline{78.73} & 59.29 & 70.35\pm16.76 \\
& AUPR ↑  & 16.60 & \textbf{64.97} & \underline{48.42} & 17.45 & 36.86\pm23.88 \\
\hline
% \multirow{3}{*}{Mean} 
% & FPR95 ↓ & 52.00 & 64.80 & 59.17 & \textbf{39.84} &- \\
% & AUROC ↑ & 73.03 & 59.30 & 66.24 & \textbf{81.50} &-\\
% & AUPR ↑  & 29.38 & 22.02 & 25.96 & \textbf{39.98} &-\\
% \hline
\end{tabular}
% }
\vspace{-2em}
\label{tab:ood1}
\end{table}

==> Table/ablation_OOD2_.tex <==
\begin{table*}[ht]
\centering
\small  % 调整字体大小
% \caption{OOD detection performance with the introduction of any two categories of \textit{atypical} data. The best results are highlighted in \textbf{bold}, and the worst results are \underline{underlined}.}
\caption{OOD detection performance using pairwise combinations of \textit{atypical} data subsets, each introducing varying degrees of semantic and visual coverage. The best results per metric are highlighted in \textbf{bold}, and the second-best results are \underline{underlined}. The symbol ``+'' indicates the introduction of auxiliary \textit{atypical} data. Abbreviations: abn = abnormal, sci = sci-fi, uni = unintentional, ani = animation.}

\vspace{0.5em}
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{c|c|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X|c}
\toprule
\footnotesize \textbf{Test Sets} & 
\footnotesize \textbf{Metric} & 
\footnotesize +abn\_sci & 
\footnotesize +abn\_uni & 
\footnotesize +abn\_ani & 
\footnotesize +ani\_sci & 
\footnotesize +ani\_uni & 
\footnotesize +sci\_uni & 
\footnotesize \makecell{Mean ± Std Dev} \\
\midrule
\multirow{3}{*}{HMDB51~\cite{kuehne2011hmdb}} 
& FPR95 ↓ & 81.86 & \underline{78.36} & 80.72 & 82.06 & 79.06 & \textbf{76.77} & 79.81\pm2.10 \\
& AUROC ↑ & 65.50 & 65.77 & 66.63 & 66.03 & \underline{68.09} & \textbf{69.97} & 67.00\pm1.72 \\
& AUPR ↑  & \underline{29.38} & 23.39 & 28.40 & \textbf{30.49} & 25.93 & 28.67 & 27.71\pm2.60 \\
\hline
\multirow{3}{*}{MiT-v2~\cite{monfort2019moments}} 
& FPR95 ↓ & 79.98 & 68.26 & 78.49 & 79.70 & \textbf{61.40} & \underline{64.83} & 72.11\pm8.27 \\
& AUROC ↑ & 63.89 & 73.46 & 67.23 & 65.35 & \textbf{75.30} & \underline{74.87} & 70.02\pm5.11 \\
& AUPR ↑  & 24.36 & 31.82 & 26.91 & 25.36 & \underline{32.94} & \textbf{33.16} & 29.09\pm4.00 \\
\hline
\multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-surreal}} 
& FPR95 ↓ & 75.99 & 48.32 & 73.31 & 74.11 & \textbf{47.32} & \underline{48.29} & 61.22\pm14.54 \\
& AUROC ↑ & 64.54 & \textbf{83.28} & 67.74 & 65.95 & \underline{82.94} & 82.22 & 74.45\pm9.23 \\
& AUPR ↑  & 22.26 & \textbf{44.81} & 25.18 & 23.31 & \underline{44.69} & 44.14 & 34.07\pm11.52 \\
\hline
\multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-theatre}} 
& FPR95 ↓ & 75.96 & 81.27 & \underline{57.40} & \textbf{41.13} & 58.72 & 64.70 & 63.20\pm14.37 \\
& AUROC ↑ & 69.89 & 56.26 & \underline{82.45} & \textbf{91.18} & 73.34 & 70.19 & 73.89\pm11.94 \\
& AUPR ↑  & 31.75 & 16.73 & \underline{52.84} & \textbf{73.82} & 28.64 & 26.72 & 38.42\pm21.02 \\
\bottomrule
\end{tabularx}
}
\label{tab:ood2}
\vspace{-1em}
\end{table*}

==> Table/ablation_OOD3_.tex <==
\begin{table}[H]
\centering
\small
\caption{OOD detection performance with the introduction of any three categories of \textit{atypical} data. + indicates the introduction of auxiliary \textit{atypical} data.  $abn$ denotes [\textit{atypical}]-{abnormal}, $ani$ denotes [\textit{atypical}]-animation, $sci$ denotes [\textit{atypical}]-sci-fi, and $uni$ denotes [\textit{atypical}]-unintentional. The best results per metric are highlighted in \textbf{bold}, and the second-best results are \underline{underlined}.}
\vspace{0.5em}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cccc|c}
\hline
\makecell{Test sets} & Metric & +$ani\_abn\_sci$ & +$ani\_abn\_uni$ & +$ani\_sci\_uni$ & +$abn\_sci\_uni$ & \makecell{Mean ± Std Dev} \\
\hline
\multirow{3}{*}{\shortstack{{HMDB51}\\~\cite{kuehne2011hmdb}}}  
& FPR95 ↓ & 80.53 & \textbf{73.21} & \underline{75.68} & 76.51 & 76.48 \pm 3.04 \\
& AUROC ↑ & 66.84 & 67.19 & \textbf{69.44} & \underline{67.77} & 67.81 \pm 1.15 \\
& AUPR ↑  & \textbf{29.81} & 24.49 & \underline{27.79} & 25.61 & 26.93 \pm 2.36 \\
\hline
\multirow{3}{*}{
\shortstack{{MiT-v2}\\~\cite{monfort2019moments}}} 
& FPR95 ↓ & 77.76 & 68.28 & \textbf{65.06} & \underline{66.24} & 69.34 \pm 5.77 \\
& AUROC ↑ & 67.12 & 72.64 & \underline{73.89} & \textbf{73.98} & 71.91 \pm 3.25 \\
& AUPR ↑  & 25.85 & 30.40 & \underline{31.59} & \textbf{32.35} & 30.05 \pm 2.91 \\
\hline
\multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-surreal}} 
& FPR95 ↓ & 71.84 & \underline{50.31} & \textbf{48.93} & 52.17 & 55.81 \pm 10.77 \\
& AUROC ↑ & 66.89 & 81.35 & \textbf{83.42} & \underline{81.44} & 78.28 \pm 7.65 \\
& AUPR ↑  & 23.63 & 41.54 & \textbf{46.17} & \underline{42.03} & 38.34 \pm 10.03 \\
\hline
\multirow{3}{*}{\shortstack{{\textnormal{[}\textit{atypical}\textnormal{]}} \\-theatre}} 
& FPR95 ↓ & \textbf{58.83} & 67.08 & \underline{63.72} & 69.30 & 64.73 \pm 4.55 \\
& AUROC ↑ & \textbf{80.94} & 70.68 & \underline{74.13} & 67.49 & 73.31 \pm 5.76 \\
& AUPR ↑  & \textbf{51.23} & 26.80 & \underline{34.04} & 23.60 & 33.92 \pm 12.34 \\
\hline
\end{tabular}
}
\label{tab:ood3}
\end{table}
